Semantic RGB--Depth Based Surgical Skill Assessment in Microscopic Stereo Videos

Objective assessment of microsurgical technical skill is essential for competency-based training and quality assurance, yet existing video-based approaches predominantly rely on RGB images and therefore overlook the 3D spatial relationships that characterize instrument-anatomy interactions. Although stereo operating microscopes provide complementary depth information, conventional stereo matching algorithms can produce sparse and unreliable depth estimates under high-magnification imaging conditions, limiting their use for automated skill assessment. This work presents a semantic RGB-Depth framework for surgical skill assessment from microscopic stereo videos. A regression-based depth fusion method combines sparse metric stereo depth with dense monocular depth estimates to generate a dense geometric representation of the surgical scene. This representation is integrated with semantically decomposed RGB streams corresponding to individual surgical instruments and surrounding anatomy. A hierarchical attention architecture jointly encodes these streams to capture discriminative patterns of instrument use and instrument-anatomy interaction across surgeons at different training levels. The framework was evaluated on 33 ex vivo transoral microlaryngeal procedures performed by six surgeons, comprising attending surgeons and surgical residents, using leave-one-surgeon-out cross-validation. The proposed semantic RGB-Depth model achieved an F1 score of 0.938 for skill-level classification, compared with 0.696 for semantic RGB and 0.929 for semantic depth. These results suggest that geometric information can improve automated surgical skill assessment from microscopic stereo videos. The learned spatial, temporal, and semantic attention patterns also support qualitative examination of the scene regions, video segments, and semantic streams emphasized by the model.

==> related_work.tex <==
\section{Related Work}\label{sec:Related_Work}

This work is related to surgical instrument motion analysis, depth reconstruction from microscopic video, and video-based surgical skill assessment. Unlike external-camera motion analysis methods~\cite{pecoraro2025computer}, we focus on microscopic surgical video, where instrument-centered visual, depth, and trajectory cues must be inferred directly from the operative view.

\subsection{Surgical instrument motion and 3D reconstruction}

Instrument motion analysis methods can be broadly divided into marker-based and markerless approaches. Marker-based systems attach physical markers to instruments and can provide accurate tracking under controlled conditions. For example, Siyar et al.~\cite{siyar2020tremor} quantified physiological tremor in a simulated tumor resection task, while Franco et al.~\cite{franco2024tracking} compared color-marker-based stereoscopic tracking with a YOLOv8-based instrument identification method for microsurgery. Other task-specific systems have also been used to evaluate microsurgical performance and robotic assistance~\cite{conroy2014video,akst2018robotic}. Although effective, these approaches often require specialized hardware, modified instruments, or constrained experimental setups.

Markerless methods estimate instrument motion directly from surgical video and are therefore more compatible with routine surgical workflows. Prior studies have investigated video-based motion analysis in microsurgery, including tremor evaluation during retinal injection~\cite{li2024tremor} and semi-automated instrument motion analysis using proprietary tools~\cite{kanumuri2019semiautomated}. However, many of these methods operate primarily in the two-dimensional image plane. While 2D tracking captures lateral motion, it provides limited access to out-of-plane movement and depth-dependent tool interaction, which are important for analyzing instrument behavior under a microscope.

Stereo microscopic video offers a potential route to metric 3D motion analysis, but reliable dense depth estimation remains challenging. Surgical microscopes are difficult to calibrate and rectify precisely, and stereo correspondence can be degraded by narrow baseline geometry, weak texture, specular reflections, occlusions, and limited depth of field. As a result, stereo methods can provide useful sparse metric measurements but may fail to recover a complete dense representation of the surgical foreground. Monocular depth estimation provides complementary dense structure, and recent models such as Depth Anything produce robust relative depth estimates across diverse scenes~\cite{yang2024depthanything,yang2024depthanythingv2}. However, monocular depth is scale-ambiguous and must be metrically aligned before it can support quantitative 3D trajectory analysis.

Recent general-purpose vision foundation models also provide useful components for video-based reconstruction. Segment Anything enables prompt-based object segmentation~\cite{kirillov2023segment}, CUTIE propagates object masks across video frames~\cite{cheng2024putting}, and CoTracker estimates temporally consistent point correspondences~\cite{karaev2023cotracker}. These models were not developed specifically for surgical foreground reconstruction, but their outputs can provide masks, tracks, and dense relative depth cues. In this work, we use them as modular components and combine their outputs with sparse stereo measurements to obtain metrically grounded 3D instrument trajectories. Compared with prior foreground-conditioned monocular depth reconstruction that aligns relative depth to registered preoperative anatomy~\cite{mao2026speak}, our approach uses stereo measurements from the microscope as the metric reference, avoiding dependence on preoperative CT or rigid anatomy registration.

\subsection{Video-based surgical skill assessment}

Automated surgical skill assessment has been studied using video, kinematic data, and multimodal cues. Funke et al.~\cite{funke2019video} showed that end-to-end spatiotemporal networks can infer surgical skill from video clips. Hira et al.~\cite{hira2022video} used temporal instrument keypoint models, while Fathollahi et al.~\cite{fathollahi2022video} studied long-term tool tracking from surgical video. Liu et al.~\cite{liu2021towards} proposed a multi-cue framework for skill assessment, and Wan et al.~\cite{wan2024spatiotemporal} introduced a spatial-temporal attention model for intraoperative skill assessment. Recent microsurgical studies further suggest that instrument motion and foreground deformation provide complementary indicators of technical performance~\cite{sugiyama2025ai}.

Despite these advances, many video-based skill assessment models rely on two-dimensional image measurements, task-specific tracking outputs, or raw full-frame appearance. This can make the learned representation sensitive to illumination, tissue appearance, camera viewpoint, field of view, or experimental setup, especially when datasets are small. Such nuisance cues are problematic when the goal is not only to classify skill level, but also to identify interpretable motion patterns that are meaningful for surgical training.

Our work addresses this limitation by combining reconstructed 3D instrument trajectories with instrument-centered RGB-D visual descriptors. Rather than learning directly from full-frame RGB-D video, we train a U-Net-based semantic segmentation model~\cite{ronneberger2015u} on RGB-D clips to segment and classify surgical instruments, and then use its predicted masks and frozen encoder features as an appearance-controlled visual representation. These segmentation-derived descriptors are fused with 3D trajectory-window features in a temporal model with branch-specific outputs, multiple-instance learning, and attention to classify expert--resident skill and localize discriminative procedural windows.


\begin{comment}
\begin{enumerate}
    %Microsurgical skills of trainee surgeons have been subjectively evaluated due to the lack of technological tools.
    % Surgical skill methods can be broadly classified as per input data type: kinematic, vidoe, multi-modal. Among these video based methods can be broadly generalizable for both robotic and non-robotic procedures. 
    % Surgical videos capture a rich information of the surgical field that can be used to assess intraoperative surgical technical skill.
    \item Prior studies for video-based surgical skill assessment can be categorized into two categories \cite{wan2024spatiotemporal}: a) end-to-end approaches for mapping of RGB video images to surgical skill, for instance by stacking CNNs for short-term spatial feature extraction and LSTMs for long-term temporal feature modeling to extract spatial-temporal features to predict surgical skill; b) multi-stage approach\cite{lavanchy2021automation,hira2022video} that first capture localized contextual information e.g., instrument motion  followed by temporal prediction of instrument motion using a temporal convolutional network.
    %methods that explicitly acquire specific features e.g., instrument motion \cite{lavanchy2021automation,hira2022video}; and c) methods that use localized contextual information about instruments, anatomy, or their interactions. 
    \item Most existing methods follow an end-to-end approach that provide little details about what motion or appearance information is captured.
    \item Most methods perform the global operation over the spatial features that compresses all the information together in the spatial scale without distinction \cite{li2022surgical}. This global operation ignores the semantics variance of different features. As a result, the temporal networks could hardly model the temporal relationship of the local features in different spatial parts separately. Both the motion of different tools and interactions between tools and tissue across time are important for the assessment. 
    \item Similar to multi-modal approach~\cite{liu2021towards}, our framework adopts a multi-path design, in which multiple paths are organized in parallel such that each path concentrates on one skill aspect. However, we employ this approach to semantic video streams in contrast to multi-modal streams.
    %Our objective of this work is to test the hypothesis that explicitly supervising attention improves network performance and generalizability for video-based approach of surgical technical skill. We expect that supervising spatial attention would allow the network to focus on the most informative streams in the images and improve the robustness against spurious features from irrelevant regions. Thus, it addresses the challenges posed by dataset shifts to generalizability of the algorithms. 
    %
    %Stereo microscopic video offers a potential route to metric 3D motion analysis, but reliable dense depth estimation remains challenging. Surgical microscopes are difficult to calibrate narrow baseline geometry, weak texture, specular reflections, occlusions, and limited depth of field. As a result, stereo methods can provide useful sparse metric measurements but may fail to recover a complete dense representation of the surgical foreground. Consequently, the video based asseesment is restrcited to 2D~\cite{cho2024tremor}
    %
    \item Instrument motion analysis in surgical videos~\cite{conroy2014video,kanumuri2019semiautomated}
    \item conventional calibration methods are unsuitable for surgical microscopes because of their narrow depth of focus at high magnifications~\cite{jeung2023intraoperative,ayaz2017survey,ha2024target}
    \item \cite{siyar2020tremor} investigation of the application of a VR platform for the quantitation of physiological tremor during a tumor resection task
    \item \cite{franco2024tracking} compared two methods for tracking 3D movement during microsurgery: Mitracks3D, a stereoscopic tracker using color-marked instruments, and a deep learning method for instruments identification based on YOLOv8. Mitracks3D as a stereoscopic exoscope system for tracking and analyzing maneuvers in microsurgery as a modality to enhance surgical training,
    \item \cite{narasimhan2025monocular} developed method for monocular videos using Florence2 and Segment Anything 2 (SAM2)—for zero-shot 2D localization of tooltip coordinates using a monocular video input. Localization predictions are refined through supervised training of the YOLOv11 segmentation model to enable real-time applications. The depth estimation model Metric3D computes the relative depth and provides tooltip camera coordinates
    \item video-based tremor analysis~\cite{friedrich2024validation} employed Mediapipe pose tracking algorithm, for comprehensive tremor analysis. We evaluate its capability to track hands in clinical standard videos of postural and kinetic tremor assessments and use the resulting time series data to compute both fundamental and advanced tremor features.
    \item \cite{li2024tremor} evaluation of tremors during retinal injection surgery
    \item Previous works on activity recognition rely on temporal models to capture long-term dependencies among activities, ranging from RNN~\cite{}, TCN~\cite{lea2017temporal}, graph neural networks~\cite{}, to transformers~\cite{}. Multi-stage temporal models~\cite{farha2019ms,li2020ms} have shown to perform better by employing incremental refining
    \item skill~\cite{liu2021towards,li2022surgical,anastasiou2023keep,ding2023sedskill}, tremor~\cite{liu2023vision}
    \item Instrument motion analysis in surgical videos~\cite{conroy2014video,kanumuri2019semiautomated}
    \item recent works propose video- or hybrid-based methods, leveraging spatial and temporal feature encoders to extract discriminative features or by using multi-task architectures 
    
\end{enumerate}
\end{comment}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{model_archetecture.png}
\caption{
Architecture of the proposed semantic RGB--depth framework for surgical skill assessment. 
Each trial is decomposed into three semantically aligned streams corresponding to the grasper, scissors, and anatomy/background regions. 
Within each stream, RGB and depth features are projected into a common latent space, fused, and temporally encoded using an independent dilated TCN. 
The encoded stream representation $\mathbf{h}_{t,k}$ is processed by a local score head to produce frame-level skill evidence $s_{t,k}$. 
A stream-specific temporal-attention branch learns $\alpha_{t,k}$, normalized over time within each stream, and forms the auxiliary local skill prediction
$\hat{y}_{k}=\sum_{t=1}^{T}\alpha_{t,k}s_{t,k}$. 
For global fusion, frame-wise stream attention $\gamma_{t,k}$, normalized across streams, weights the three semantic representations at each time step. 
The resulting fused sequence is processed by a global temporal-attention module to obtain $\alpha_t$, which identifies the most informative frames across the trial. 
The final prediction is computed as
$\hat{y}=\sum_{t=1}^{T}\sum_{k=1}^{3}\alpha_t\gamma_{t,k}s_{t,k}$. 
The auxiliary stream-level regression objective encourages each semantic stream to retain independently discriminative skill information while complementing the global prediction loss.
}
    
    \label{fig:model_overview}
\end{figure*}

